More Information is Not Always Better: Connections between Zero-Sum Local Nash Equilibria in Feedback and Open-Loop Information Patterns

Non-cooperative dynamic game theory provides a principled approach to modeling sequential decision-making among multiple noncommunicative agents. A key focus has been on finding Nash equilibria in two-agent zero-sum dynamic games under various information structures. A well-known result states that in linear-quadratic games, unique Nash equilibria under feedback and open-loop information structures yield identical trajectories. Motivated by two key perspectives -- (i) many real-world problems extend beyond linear-quadratic settings and lack unique equilibria, making only local Nash equilibria computable, and (ii) local open-loop Nash equilibria (OLNE) are easier to compute than local feedback Nash equilibria (FBNE) -- it is natural to ask whether a similar result holds for local equilibria in zero-sum games. To this end, we establish that for a broad class of zero-sum games with potentially nonconvex-nonconcave objectives and nonlinear dynamics: (i) the state/control trajectory of a local FBNE satisfies local OLNE first-order optimality conditions, and vice versa, (ii) a local FBNE trajectory satisfies local OLNE second-order necessary conditions, (iii) a local FBNE trajectory satisfying feedback sufficiency conditions also constitutes a local OLNE, and (iv) with additional hard constraints on agents' actuations, a local FBNE where strict complementarity holds also satisfies local OLNE first-order optimality conditions, and vice versa.

==> sections/04_main__results.tex <==
\section{Main Results}\label{sec: main results}
In the following theorem, we show how state/control trajectories corresponding to any local FBNE policies are related to a local OLNE for the zero-sum game of the type described in \Cref{sec: Preliminaries}, i.e., containing no constraints apart from those due to the game dynamics. 
\begin{theorem}\label{theorem: main theorem}
    Consider a two-agent zero-sum dynamic game with $K$ stages and dynamics constraints. Then:
    \begin{enumerate}
        \item The controls and states corresponding to any existing local FBNE also satisfy the first- and second-order necessary conditions for a local OLNE of the game.
        \item The controls and states corresponding to any existing local OLNE also satisfy the first-order necessary conditions for a local FBNE of the game.
        \item Assume that a local FBNE of the game exists, and that the corresponding local feedback equilibrium strategies $\uifbtstar=\{\mapieq_t(x_t),~t\in [K]\},~i=1,2,$ and state trajectory  $\x(\uonefbstar_{1:K}, \utwofbstar_{1:K})=\{\x^*_1,\dots,\x^*_{K+1}\}$ satisfy the FBNE second-order sufficiency conditions. Then $\uifbtstar$ and $\x(\uonefbstar_{1:K}, \utwofbstar_{1:K})$ also constitute a local OLNE of the game.
    \end{enumerate}
\end{theorem}
\begin{proof}
    % To prove this, we show that for each agent, the feedback KKT conditions \eqref{eq: fb kkt nabla xs}-\eqref{eq: fb kkt -i feedback pol cons} \doubt{become exactly/also satisfy} the open-loop KKT conditions \eqref{eq: ol kkt nabla xt}-\eqref{eq: ol kkt dynamics cons}. Let $\x(\uonefb_{1:K}, \utwofb_{1:K})=\{\xstartime{1},\dots,\xstartime{K+1}\}$
    We prove the first part by showing that at any local FBNE of the game, the feedback policy constraints \eqref{eq: fb kkt -i feedback pol cons} are weakly active for both agents. The KKT condition for agent $-i$ corresponding to \eqref{eq: fb kkt nabla xfinal} is
    \begin{equation}
    \nabla_{\x_{K+1}}\lmi_{K+1}(\xstartime{K+1}) -\lambmi_K =0. \label{eq: proof mi final state kkt}
    \end{equation}
    Because the game is zero-sum, $\nabla_{\x_{K+1}}\lmi_{K+1} = - \nabla_{\x_{K+1}}\li_{K+1}$, and from \eqref{eq: proof mi final state kkt} combined with \eqref{eq: fb kkt nabla xfinal} evaluated at $\xstartime{K+1}$ we get
    \begin{equation}
        \lambmi_K = -\lambi_K. \label{eq: neg lambdas}
    \end{equation}
    Using the KKT condition \eqref{eq: fb kkt nabla umis} corresponding to agent $-i$ evaluated at time $s=K$, and \eqref{eq: neg lambdas}, we get 
    \begin{align}
        -\nabla_{\uifbtime{K}}\li_K - (\nabla_{\uifbtime{K}}f_K)^\top \lambi_{K}- \psimapmik = ~0. \label{eq: mi umis kkt feedback}
    \end{align}
    Using \eqref{eq: fb kkt nabla uis} evaluated at time $s=K$ and \eqref{eq: mi umis kkt feedback} we get
    \begin{align}
        \psimapmik = 0. \label{eq: psimapmik = 0}
    \end{align}
    Similarly, for the Lagrange multiplier for agent $i$ in the KKT conditions of agent $-i$, we get
    \begin{align}
        \psimapik = 0. \label{eq: psimapik = 0}
    \end{align}
    Using the KKT condition \eqref{eq: fb kkt nabla xs} for both agents $i, -i$ evaluated at time $s=K$, \eqref{eq: neg lambdas}, \eqref{eq: psimapmik = 0} and \eqref{eq: psimapik = 0}, we get
    \begin{align}
        \lambmi_{K-1} = -\lambi_{K-1}. \label{eq: neg lambdas cascading}
    \end{align}
    Equation \eqref{eq: neg lambdas cascading} suggests the following recursive pattern, which can be verified by continuing the previous arguments: $\lambmi_t = -\lambi_t,~\forall~t\in[K]$. This yields
    \begin{align}
        \psimap^i_t = \psimap^{-i}_t = 0~\forall~t\in T_2.\label{eq: all psi zero}
    \end{align}
    \emph{Thus, at a local FBNE, the constraints forcing both agents to play feedback policies are weakly active.} From \Cref{remark: fb ol diff} and \eqref{eq: all psi zero}, we can conclude that the local FBNE KKT conditions \eqref{eq: fb kkt nabla umis}-\eqref{eq: fb kkt nabla xs} imply the local OLNE KKT conditions \eqref{eq: ol kkt nabla xt}-\eqref{eq: ol kkt dynamics cons} and thus $\uonefbstar,~\utwofbstar,~\x(\uonefbstar_{1:K}, \utwofbstar_{1:K})$ also satisfy the first-order necessary conditions for a local OLNE. 
    \par
    Now consider the feedback second-order sufficiency conditions \eqref{eq: fb second order start}-\eqref{eq: fb second order end}. Because the feedback policy constraints are weakly active, from \Cref{remark: fb ol diff}, the condition \eqref{eq: fb second order end} can be dropped while considering the directions in the critical cone for which \eqref{eq: fb second order start} should hold. Further, we observe that the directions such that
    \begin{align}
    d_{\umit} & =0  \label{eq: fb reduced second order umit}\\
    d_{\xtone} - \nabla_{\uit}f_s d_{\uit} &= 0, \label{eq: fb reduced second order xt}\\
    d_{\xsone} - \nabla_{\xs}f_s d_{\xsone}- \nabla_{\uis}f_s 
        d_{\uis}
     &= 0~\forall~ s\in T_{t+1}, \label{eq: fb reduced second order xs}
    %d_{\umis} - \nabla_{\xs}\mapmis d_{\xs} &= 0~\forall~ s\in T_{t+1}.
    \end{align}
    all lie in the directions in the critical cone defined by \eqref{eq: fb second order xs}, \eqref{eq: fb second order xt}. We observe that \eqref{eq: fb reduced second order umit}-\eqref{eq: fb reduced second order xt} when applied to \eqref{eq: fb second order start} exactly yield the open-loop second-order sufficiency conditions \eqref{eq: ol second order start}-\eqref{eq: ol second order end}.  \emph{Thus the directions in the open-loop critical cone are a subset of the directions in the feedback critical cone.} From \Cref{remark: fb ol diff} a similar relation holds for second order necessary conditions between feedback and open-loop settings. Because the FBNE controls/states must be satisfying the feedback second-order necessary conditions, this implies that they also satisfy the OLNE second order necessary conditions. This proves the first part of the theorem.
    \par
    To prove the second part of the theorem, let a local OLNE exist and $\uoneolstar_{1:K}, \utwoolstar_{1:K}, \x^{*,OL}_{1:K+1}:=\x(\uoneolstar_{1:K}, \utwoolstar_{1:K})$ denote the corresponding controls and states. Thus, $\uoneolstar_{1:K}, \utwoolstar_{1:K}, \x^{*,OL}$ satisfy the open-loop KKT conditions \eqref{eq: ol kkt nabla xt}-\eqref{eq: ol kkt dynamics cons}. Then it is trivial to observe that $\uoneolstar_{1:K}, \utwoolstar_{1:K}, \x^{*,OL}$ also satisfy the feedback KKT conditions \eqref{eq: fb kkt nabla umis}-\eqref{eq: fb kkt nabla xs} for the choice of feedback policy constraints $\psimap^i_t = \psimap^{-i}_t = 0~\forall~t\in[K]$. Note that the open-loop trajectory also satisfies \eqref{eq: fb kkt -i feedback pol cons}, because the open-loop controls are derived by solving the KKT conditions backwards in time, which implies that the local OLNE controls satisfy \eqref{eq: FBNE def}.
    \par
    For the third part of the theorem, if $\uonefbstar,~\utwofbstar,~\x(\uonefbstar_{1:K}, \utwofbstar_{1:K})$ satisfy the feedback second-order sufficiency conditions \eqref{eq: fb second order start}-\eqref{eq: fb second order end}, from the discussion above, we can conclude that $\uonefbstar,~\utwofbstar,~\x(\uonefbstar_{1:K}, \utwofbstar_{1:K})$ also satisfy the second-order sufficiency conditions of (and thus constitute) a local OLNE of the game.
\end{proof}
